Federated learning with differential privacy and an untrusted aggregator

Federated learning for training models over mobile devices is gaining popularity. Current systems for this task exhibit significant trade-offs between model accuracy, privacy guarantee, and device efficiency. For instance, Oort (OSDI 2021) provides excellent accuracy and efficiency but requires a trusted central server. On the other hand, Orchard (OSDI 2020) provides good accuracy and the rigorous guarantee of differential privacy over an untrusted server, but creates huge overhead for the devices. This paper describes Aero, a new federated learning system that significantly improves this trade-off. Aero guarantees good accuracy, differential privacy over an untrusted server, and keeps the device overhead low. The key idea of Aero is to tune system architecture and design to a specific set of popular, federated learning algorithms. This tuning requires novel optimizations and techniques, e.g., a new protocol to securely aggregate updates from devices. An evaluation of Aero demonstrates that it provides comparable accuracy to plain federated learning (without differential privacy), and it improves efficiency (CPU and network) over Orchard by up to $10^5\times$.

==> GNUmakefile <==
MAIN = paper.tex

BASE      := $(basename $(MAIN))
SRCEXT    := $(patsubst $(BASE).%,%,$(MAIN))
XFIGS     := $(wildcard fig/*.fig)
DIAFIGS   := $(wildcard fig/*.dia)
SVGFIGS   := $(wildcard fig/*.svg)
CORELFIGS := $(wildcard fig/*.cdr)
CORELPDF  := $(patsubst fig/%.cdr, fig/%.pdf, $(CORELFIGS))

TEXFIGS   := $(patsubst fig/%.fig, fig/%.tex, $(XFIGS)) # $(DIAFIGS:.dia=.tex)
BINFIGS   := $(patsubst fig/%.fig, fig/%.pdf, $(XFIGS)) \
    	     $(patsubst fig/%.dia, fig/%.pdf, $(DIAFIGS)) \
#    	     $(patsubst fig/%.svg, fig/%.pdf, $(SVGFIGS))  


STYLINK	  := $(notdir $(wildcard ../*.sty))
STYFILES  := $(sort $(STYLINK) $(wildcard *.sty))
TEXFILES  := $(sort $(MAIN) $(wildcard *.tex) $(STYFILES) $(TEXFIGS))

BIBFILES  := $(wildcard bib/*.bib)

RSLTS     := $(wildcard rslt/*.json)
JGRAPHS   := $(wildcard jgraph/*.j)
GGRAPHS   := $(wildcard gp/*.gp)
BARGRAPHS := $(wildcard gp/*.sh)
BAREPS    := $(patsubst gp/%.sh, graphs/%.eps, $(BARGRAPHS))
BARGRAPHDRIVER := $(patsubst %, gp/%, barchart barchart-stacked)
# Credit for the sed command goes to stackoverflow.com user Zsolt Botykai
TEXTABLES := $(shell grep graph_file graph_gen.json | cut -d\" -f4 | sed ':a;N;$!ba;s/\n/ /g')

GRAPHS    := $(patsubst jgraph/%.j, graphs/%.pdf, $(JGRAPHS)) \
    	     $(patsubst gp/%.gp, graphs/%.pdf, $(filter-out gp/style.gp, $(GGRAPHS))) \
	     $(patsubst gp/%.sh, graphs/%.pdf, $(BARGRAPHS))

DATA      := $(wildcard dat/*.dat)

# LATEX \\def\\noeditingmarks{} \input
LATEX     = pdflatex -shell-escape #\\nonstopmode\\input
BIBTEX    = bibtex -min-crossrefs=1000
PS2PDF    = ps2pdf
RSLT2GRAPH = rslt_to_graphs.py
RSLT2GRAPHCONFIG = graph_gen.json
PYTHON    = python

SHA = shasum

export TEXINPUTS=".:./style:";

all: $(BASE).pdf

data-stamp: $(RSLTS) $(RSLT2GRAPH) $(RSLT2GRAPHCONFIG) $(wildcard *skeleton*)
# Depot way (also used in speak-up):
#	for i in `ls scripts/*.py scripts/*.pl scripts/*.sh`; do $$i; done
	mkdir -p dat; mkdir -p graphs
	$(PYTHON) $(RSLT2GRAPH) $(RSLT2GRAPHCONFIG)
	touch $@

# to include an xfig with embedded latex, you include the *tex* file:
# \begin{figure}
#    \input{foo}
# \end{figure}
#  where fig/foo.fig is an xfig file that you created with embedded latex.
%.pdf %.tex: %.fig
	fig2dev -L pdftex -p1 $< > $*.pdf
	fig2dev -L pdftex_t -p $*.pdf $< > $*.tex

%.pdf: %.eps
	perl -ne 'exit 1 unless /\n/' $< \
		|| perl -p -i -e 's/\r/\n/g' $<
	epstopdf --outfile=$@ $<

%.pdf: %.gif
	convert $< $@

%.tex: %.dia
	unset DISPLAY; dia -n -e $@ $<

# dirt-simple rule to build graphs. depends on gnuplot file printing its
# output (the PDF file) to stdout
graphs/%.pdf: gp/%.gp data-stamp 
	gnuplot < $< > $@

graphs/%.pdf: jgraph/%.j data-stamp 
	@rm -f $@~
	jgraph $< > $@~
	mv -f $@~ $@

graphs/%.pdf: gp/%.sh $(BARGRAPHDRIVER) data-stamp
	@rm -f $@~
	$< 

# convert SVG figures to PDF
#fig/%.pdf: fig/%.svg
#	@rm -f $@~
#	inkscape --export-pdf=$@~ $<
#	mv -f $@~ $@

$(STYLINK):
	rm -f $@
	ln -s ../$@ .

RERUN = egrep -q '(^LaTeX Warning:|\(natbib\)).* Rerun' $*.log
UNDEFINED = egrep -q '^(LaTeX|Package natbib) Warning:.* undefined' $*.log
 
# So you can "setenv ALWAYS yes" instead of butchering the Makefile...
ifneq ($(ALWAYS),)
ALWAYS = always
endif

$(BASE).pdf: %.pdf: %.$(SRCEXT) $(TEXFILES) $(BIBFILES) \
				$(BINFIGS) $(GENTEX) $(TEXFIGS)	\
				$(ALWAYS) $(TEXTABLES) $(CORELPDF) $(GRAPHS)
	test ! -s $*.aux || $(BIBTEX) $* || rm -f $*.aux $*.bbl
	$(LATEX) $< || ! rm -f $@
	if $(UNDEFINED); then \
		$(BIBTEX) $* && $(LATEX) $< || ! rm -f $*.bbl $@; \
	fi
	! $(RERUN) || $(LATEX) $< || ! rm -f $@
	! $(RERUN) || $(LATEX) $< || ! rm -f $@
	touch $*.dvi
	test ! -f .xpdf-running || xpdf -remote $(BASE)-server -reload

%.pdf: %.ltx
	$(LATEX) $< || !rm -f $@
	! $(RERUN) || $(LATEX) $< || ! rm -f $@
	! $(RERUN) || $(LATEX) $< || ! rm -f $@

$(TEXTABLES): $(RSLT2GRAPH) $(RSLT2GRAPHCONFIG) $(RSLTS) data-stamp

DIST = GNUmakefile $(filter-out $(GENTEX) $(TEXFIGS), $(TEXFILES)) \
	$(XFIGS) $(DIAFIGS) \
	$(JGRAPHS) $(GGRAPHS) $(BARGRAPHS) \
	$(BARGRAPHDRIVER) \
	$(RSLTS) \
	$(BIBFILES)
dist: $(BASE).tar.gz
$(BASE).tar.gz: $(DIST)
	tar -chzf $@ -C .. \
		$(patsubst %, $(notdir $(PWD))/%, $(DIST))

PREVIEW := $(BASE)
preview: $(PREVIEW).pdf
	if test -f .xpdf-running; then			\
		xpdf -remote $(BASE)-server -quit;	\
		sleep 1;				\
	fi
	touch .xpdf-running
	(xpdf -remote $(BASE)-server $(PREVIEW).pdf; rm -f .xpdf-running) &

show: $(BASE).pdf
	xpdf -fullscreen $(BASE).pdf

osx: $(BASE).pdf
	open $(BASE).pdf

anon: $(BASE)-anon.pdf

double:
	for i in $(TEXFILES); do perl double.pl $$i; done

# stupid hack to anonymize a PDF. it's maybe ridiculous that this
# works.
$(BASE)-anon.pdf: $(BASE).pdf
	$(PS2PDF) $< $@

EXTRAIGNORE = '*~' '*.aux' '*.bbl' '*.blg' '*.log' '*.dvi' '*.bak' '*.out' 
ignore:
	rm -f .gitignore
	(for file in $(EXTRAIGNORE); do \
		echo "$$file"; \
	done; \
	for file in .xpdf-running \
			$(BASE).tar.gz \
			$(GENTEX) $(TEXFIGS) $(BINFIGS) $(GRAPHS) \
			$(BASE).ps $(BASE).pdf; do \
		echo "/$$file"; \
	done) | sort > .gitignore
	git add .gitignore

clean: 
	rm -f $(BASE).ps $(BASE).pdf $(BASE).tar.gz
	rm -f $(TEXFIGS) $(BINFIGS) $(GRAPHS) $(TEXTABLES)
	rm -f $(GENTEX)
	rm -f $(DATA)
	rm -f *.dvi *.aux *.log *.bbl *.blg *.lof *.lot *.toc *.bak *.out
	rm -f *~ *.core core
	rm -f plot.plt
	rm -f $(BAREPS)
	rm -f data-stamp

always:
	@:

.PHONY: install clean all always ignore preview show osx dist 

spell:
	make clean
	for i in $(wildcard *.tex); do aspell -p ./aspell.words -c $$i; done


==> design-old.tex <==
\section{Design of \sys}
\label{s:design}

We go over the design details of \sys
phase-by-phase, while highlighting the challenges
and key design choices and techniques for each phase.
%



\subsection{Setup phase}
\label{s:design:setup}

Much of \sys's setup phase is similar to Orchard. 
During this phase, \sys (i)
    samples
    the master committee using a sortition protocol [cite], which then
    (ii) receives and validates inputs for the round
     (i.e., receives model parameters $\theta^t$ for the current round $t$,
the device selection probability $q$, 
noise scale $z$, and clipping bound $S$, and generates
    new values of the DP parameters $\epsilon, \delta$),
    and (iii) generates keys for cryptographic 
    primitives (\S\ref{s:protocoloverview}).
We do not focus on the first two pieces here to avoid repetition with Orchard, but 
    include them
    in the supplementary material for completeness [fwdptr].
Instead, the
    key challenge in \sys is the overhead of key generation.%

Recall that Orchard uses MPC among the master committee members to generate keys such 
that even if the members of the committee that are malicious collude,
they cannot recover the keys. The overhead of this MPC is high: $\approx$1~GiB of 
network transfers and 180 seconds of \cpu time per committee device. How can this overhead be reduced?


One idea [cite] is to reuse the keys across rounds rather than generate them fresh 
for each round. Indeed, this is what \sys does: the master committee in 
round 1 generates the keys and 
shares them with the committee for the next round, and this committee then shares the keys with the committee for the third round, and so on. 
But one has to be careful.

Consider the following attack. 
Say that the malicious aggregator receives a victim device's update $Enc(pk, \Delta_{k}^{t})$ 
and a ZK-proof $z$ in round $t$. 
Then, in the next round $t+1$, 
the aggregator colludes with the malicious devices to use $Enc(pk, \Delta_{k}^{t}), z$ as their update. 
In round $t+1$, no error will be reported as the ciphertext is valid; 
however, the attack will violate differential privacy as
the victim device's input will not satisfy the required clipping bound $S$ in round $t+1$ 
due to its many copies 
(\S\ref{s:overview:dpfedavg}). Orchard does not suffer from this attack as it 
generates fresh keys in each round.

Thus, \sys must apply the reuse-of-keys idea with care. 
\Sys adjusts the generate and add phases [fwdptrs] to prevent 
cipertexts generated during one round from being used
in another round; we are not in a position yet to describe these changes, but we will
detail them shortly when we describe these phases [fwdptr].
Meanwhile, 
    the changes in the setup phase are the following: 
    for the AHE secret key, \sys implements an efficient verifiable secret redistribution
    scheme~\cite{gupta2006extended}% 
    such that committee members at round $t+1$ 
    can securely obtain the relevant shares of the key 
from the committee at round $t$.
For the public keys (AHE public key, and both the public proving and verification keys for the ZK-proof scheme),
the committee for round $t$ signs and uploads them to the bulletin board, and
the committee for round $t+1$ downloads them from the board.

The savings by switching from key generation to key resharing are substantial.
While the MPC solution incurs $\approx$1~GiB of network transfers and 120 seconds
of \cpu time per device, 
key resharing requires 125~MiB and 187 seconds, respectively ($\approx$ 20$\times$ lower).%












\subsection{Generate phase}
\label{s:design:generate}


Recall that during this phase 
(i) \sys must pick a subset of devices
to generate updates to the model parameters,
(ii) the DP-noise committee must generate
Gaussian noise for differential privacy, 
and (iii) both types of devices must 
encrypt their generated data (updates and noise).
The key goal in these tasks is efficiency.

\emparagraph{Device sampling.}
One design option is to ask the aggregator to sample devices for a round from the entire set of devices. 
The problem with this option is that the (malicious) aggregator may not choose devices uniformly as required by DP-FedAvg (line~\ref{l:dpfedavg:sampleclients} in Figure~\ref{f:dpfedavg}), thereby introducing bias. This bias
would make \sys deviate from its differential privacy guarantee.% 
An alternative is to ask the devices
to sample themselves with probability $q$ (again, as required by DP-FedAvg). But then malicious clients
may participate in training more than expected (e.g., in every round), which would allow them to 
significantly affect model accuracy. Thus, \sys adopts a design in which devices sample themselves while
the aggregator verifies the sampling.

For now, assume that $B^{t}$ is a source of
randomness that is publicly verifiable. Then, each device $k$
with public key $\pi_k$ computes 
$PRG(\pi_i || B^{t})$, , where $PRG$ is a pseudorandom generator 
such as \textred{[fill in with cites]}. The device then
scales the PRG output to a value between 0 and 1, and checks if the result is less than $q$. 
For instance, if the PRG output is 8 bytes,
then it divides this number by $2^{64} - 1$.
If selected, the device runs the $\userupdate$ procedure
(line~\ref{l:dpfedavg:userupdate} in Figure~\ref{f:dpfedavg}).

The question now is how can \sys arrange $B^{t}$. We do not specify 
the details here, but $B^{t}$ is the same per-round public random 
value that is used in the sortition protocol to form committees for 
the round.



%
%

\emparagraph{Gaussian noise generation.}
One option is MPC, but expensive. Instead, 
each member of the DP-noise committee locally generates Gaussian noise 
without coordinating with other members.

The Gaussian distribution has the property that if an element 
sampled from $\mathcal{N}(0, a)$ is added to another element sampled from 
$\mathcal{N}(0, b)$, then the sum is a sample of $\mathcal{N}(a+b)$~\cite{truex2019hybrid,xu2019hybridalpha,dwork2006our}.
This works well for
the simple case when all $C$ committee members are honest. 
Given noise parameter  $\sigma = z \cdot S$, the devices can 
    independently compute their additive share.
That is, 
to generate samples from $\mathcal{N}(0, I \sigma^2)$ (line~\ref{l:dpfedavg:aggregateupdates} in Figure~\ref{f:dpfedavg}), each
committee member can sample its share of the noise from the distribution
$\mathcal{N}(0,I\frac{\sigma^2}{C})$.

The challenge is %
how
do we account for the $A$ malicious parties in the DP-committee?
Malicious devices may behave arbitrarily and may thus generate 
either no noise or large amounts of it. 
Adding unnecessary noise hurts accuracy, not privacy. 
In contrast, failing to add noise may violate privacy. 
We thus consider the worst case in which malicious users fail to add any noise and 
ask honest devices to compensate. 
Each honest client thus samples its noise share from the 
distribution $\mathcal{N}(0,I\frac{\sigma^2}{C - A})$. 

This algorithm generates noise cheaply; it does not require 
any expensive MPC computation between the committee members and thus scales
to a large number of model parameters.
The downside is that it may generate 
more noise than necessary, hurting accuracy. To mitigate this risk, we carefully choose
the committee size to minimize the ratio of additional work. Specifically, we choose C to keep the ratio $(C - A) / C$ close to 1 . 
For instance,
instead of picking a committee containing a few tens of devices similar to the master committee, 
we pick a somewhat larger DP-noise committee: $(A, C) = (40,
280)$.\footnote{Using a probabilistic argument for committee size selection as
before (\S\ref{s:design:setup}), 
if $f=3\%$ devices in the overall population are malicious, then 
the chances of sampling 280 devices with more than 1/7th malicious is 
$4.1 \cdot 10^{-14}$.} %


\emparagraph{Encryption and ZK-proofs.}
In the final step of the generate phase, 
devices must (i) encrypt their generated data to prevent the 
    aggregator from learning it, and (ii) 
certify that the encryption is done correctly and the data being 
encrypted is bounded. %
This approach preserves privacy
while limiting the 
    influence of malicious devices 
    on accuracy, who may otherwise supply arbitrary updates. 
For ZK-proof generation, 
    \sys uses a standard framework (\S\ref{s:impl}). The encryption logic, however, is more subtle.
     %
As we will explain shortly (\S\ref{s:design:add1}), 
    \sys must ensure  that a ciphertext generated in a round is used 
    only in that round. Thus, each device
    concatenates the round number 
to the plaintext message. 
     %



    
    


\input{fig-add-phase}
\subsection{Add phase}
\label{s:design:add1}

During the add phase, the aggregator adds Gaussian noise ciphertexts to user
update ciphertexts. Aero must ensure that a Byzantine aggregator cannot violate differential privacy by supplying incorrect (integrity) or stale (freshness) values.  %
\begin{myitemize}

%
\item \emph{Integrity.} Maintaining integrity requires the aggregator to perform four tasks.
First, the aggregator must add ciphertexts from all honest devices that contribute
    Gaussian noise shares in the generate phase.
Second, the aggregator must not allow a malicious device 
    to copy an honest device's input. 
Third, the aggregator must not change a ciphertext before adding it. 
Fourth, the aggregator must add ciphertexts correctly: the
result of adding two ciphertexts must decrypt to the sum of their plaintexts.

\item \emph{Freshness.} The aggregator
must use a ciphertext generated 
during a given round in that round only.

\end{myitemize}

\noindent To understand these requirements, consider a toy example with
two honest devices. The first device
inputs $\encplain(n)$, where $n$ is Gaussian noise, 
and the other
 inputs $\encplain(\Delta)$, where $\Delta$ is its update. 
 The aggregator cannot omit $\encplain(n)$ as
the added noise would then be insufficient to protect $\Delta$. Second, the aggregator cannot duplicate user input: adding $Enc(u)$
twice (i.e., $Enc(2u)$) could violate the clipping requirement of DP-FedAvg 
(line~\ref{l:dpfedavg:clipping} in Figure~\ref{f:dpfedavg}). Similarly, 
since an AHE scheme allows ciphertexts to be multiplied
by scalars, the aggregator could convert $\encplain(u)$ to $\encplain(k \cdot
u)$, where $k$ is a scalar. This again
breaks the clipping requirement.
Finally, freshness is needed as \sys reuses 
    encryption keys across rounds for efficiency of key generation 
    (\S\ref{s:design:setup}). 
Thus, the aggregator can
take a ciphertext generated in round $t$, multiply it with a scalar, and use it in a subsequent round, e.g., as an input
of a malicious device in round $t+1$. 

\Sys's starting point to satisfy these requirements is the commit-add-verify
verifiable aggregation protocol of Orchard~\cite{roth2019honeycrisp}. 
Unfortunately, this scheme does not guarantee freshness and imposes significant overheads on devices. \sys adapts and optimizes this scheme by making clever use of \textit{summation trees} and \textit{polynomial identity testing}, as we describe next (Figure~\ref{f:addphase}).  %

\sys proceeds as follows. In the \emph{commit} step, all
devices commit to their input ciphertexts before submitting 
them to the aggregator (line~\ref{l:addphase:generatecommitments} in
Figure~\ref{f:addphase}). The aggregator 
creates a Merkle tree of these commitments and publishes the root to the
bulletin board. These commitments ensure that a malicious device cannot copy
an honest device's input before submitting its commitment. This design also
ensures that the aggregator cannot change a device's input (the device's
input is committed before it is revealed).

In the \emph{add} step, the aggregator adds the ciphertexts via 
summation trees. Specifically, if device updates have $\ell$
ciphertexts, the aggregator creates $\ell$ summation trees, one 
per ciphertext. %
The leaf vertices of the $j$-th tree are the $j$-th ciphertexts in the devices'
inputs, while each parent is the sum of its children ciphertexts,
and the root is the $j$-th ciphertext in the aggregation result. 
Forming explicit summation trees allows devices to download parts of the tree
and inspect the
aggregator's work. 
Further, the aggregator publishes the vertices of the summation trees
on the bulletin board in the form of Merkle trees
(line~\ref{l:addphase:publishmerklesummationtrees} in Figure~\ref{f:addphase}), 
which allows an honest device to check that its input is 
not omitted.

In the \emph{verify} step, each device in the system 
selects a few summation trees (line~\ref{l:addphase:picksummationtrees} in
Figure~\ref{f:addphase}) and a few leaf and non-leaf vertices
within these trees and checks them, 
ensuring that the aggregator did not deviate
from its protocol. 
    For the leaf vertices, the 
device checks that the ciphertexts are
committed to in the commit step, and the ZK-proofs
    are valid (e.g., the first coefficient of the plaintext 
    in the ciphertexts equals the current round number). For the non-leafs, the device checks that they equal
    the sum of their children.



%
The use of summation trees---one per 
    ciphertext in a device's input---allows
\sys to scale with the number of parameters.
In more detail, \sys's protocol
    creates 
    $\ell$ summation trees, one for each ciphertext
in a device's input. 
    Further, each tree has $\approx q \cdot W$ leaf vertices, 
    where
    $q$ is the small (e.g., $10^{-5}$) device sampling probability
    in DP-FedAvg and $W$ is the total number of devices in the system.
    (So in total, the number of leaves is $q \cdot W \cdot \ell$.)
Crucially, since $W$ is large, each of the $W$ devices can verify a small number, i.e., $q \cdot \ell$, of the trees (line~\ref{l:addphase:picksummationtrees} in
Figure~\ref{f:addphase}).
    We prove in the Appendix (Appex.~\S\ref{sssec:agg}) that this small amount of verification work per device is sufficient for verifiability. 
    In contrast, 
    Orchard's protocol creates one (monolithic) summation tree whose
    each node contains $\ell$ ciphertexts. Thus, a verifier device
    downloads and verifies at least $\ell$ ciphertexts (while in \sys this is
    in the order of $q \cdot \ell$).

\subsection{Add phase: an additional optimization}
\label{s:design:add2}

Checking non-leaf vertices in the summation trees is the primary source of overhead of \sys's commit-add-verify aggregation protocol. 
Each device downloads
$s$ non-leaf vertices and their children and checks that 
a vertex equals the sum 
    of its children (line~\ref{l:addphase:verifynonleaf} in
Figure~\ref{f:addphase}; $s=5$ in our implementation).
This overhead is significant because BFV
    ciphertexts are large: 131~KiB (each
        ciphertext is
    two polynomials of $4,096$ coefficients each, and
    each coefficient is 16 bytes).



\Sys recognizes that ciphertexts can be expressed as polynomials. The validity of their sum can be checked more efficiently using a technique called polynomial identity testing (PIT)~\cite{schwartz1980fast,zippel1979probabilistic}.
This test says that given a $d$-degree polynomial $g(x)$ whose coefficients are
in a field
$\mathbb{F}$, one can test whether 
 $g(x)$ is a zero polynomial by picking a number $r\in \mathbb{F}$ 
uniformly and testing whether $g(r)==0$.
This works because a $d$-degree polynomial has at most $d$ solutions to
$g(x)==0$, and thus the probability of $g(r)==0$ for a non-zero $g(x)$ is at
most $d/|\mathbb{F}|$, which is negligible 
  when the field is large (as is the case for the field
    from which BFV ciphertext coefficients
    are sampled). 

Using PIT, \sys transforms the summation 
    trees and replaces the ciphertexts at the non-leaf vertices
    with their evaluations at a point $r$.
A device then during the ``Verify'' step  checks whether these evaluations 
    add up.
Thus, instead of downloading a ciphertext with $2 \cdot 4,096$ 
    field elements, 
    a device downloads two field elements for the two
    polynomials.
A (small) challenge in incorporating PIT 
    is the question of 
    who should generate $r$, which must be sampled
    uniformly from the coefficient field.
For this,
\sys extends
    the master committee to
    publish an $r$ to the bulletin board 
    in the add step.
This extension uses known techniques: 
        distributively 
        obtaining shares of a random number~\cite{damgard2006unconditionally}, 
   and committing to the shares before revealing them~\cite{damgaard2012multiparty}.
     


\subsection{Release phase}
\label{s:design:release}

During the release phase, \sys
    (i) forms the decryption committees,
    (ii) which then obtain shares 
    of the secret key of the AHE scheme 
    from the master committee, 
    (iii) and
decrypt the ciphertexts containing the aggregation results:
    the $\ell$ root nodes of the $\ell$ summation trees. 
\sys reuses the same sortition protocol to form the decryption committees (\S\ref{s:design:setup}) and
secure secret share redistribution scheme to share the secret key (\S\ref{s:design:setup}). We focus here on 
    how a committee decrypts a ciphertext.
    \sys's key contribution is in its securely pushing most of the work including the addition of DP noise outside of MPC, and tailoring MPC for the remaining work. In contrast, Orchard decrypts the ciphertexts and then adds noise for DP in generic MPC and thus incurs huge overhead.


%
%
\sys's ciphertext decryption follows the multi-key BFV scheme~\cite{chen2019efficient} and consists of two phases: a partial decryption
    step which computes an approximation of the plaintext message, 
    and a rounding step that converts the approximation into the exact 
    plaintext.
    A BFV ciphertext is a tuple 
    of polynomials $(c1, c2)$ (\S\ref{s:design:add2}). 
    The partial decryption step computes 
        $c2 - c1 \cdot skEnc$ (where $skEnc$ is the private key), which 
    equals $m/\gamma + e_{small}$, where
    $m$ is the plaintext message, $\gamma \ll 1$ is a public
    parameter, and $e_{small}$ is an error polynomial 
    with a small norm.
The rounding step then multiplies
        $m/\gamma + e_{small}$ with $\gamma$ and rounds each
        coefficient of the output polynomial 
    to the closest integer. The term $e_{small} \cdot \gamma$ 
    vanishes on rounding, leaving $m$ as the output.
        
To build intuition, first consider an insecure scheme:
each committee member computes and sends 
$c1 \cdot [skEnc]$ to the aggregator, 
where $[skEnc]$ is the committee member's share of the secret key. 
The aggregator adds these shares to obtain
$c1 \cdot skEnc$. This scheme is efficient as a committee member
performs local computations only. However, it is insecure because
the aggregator learns $c1 \cdot skEnc$ and thus $skEnc$.
\Sys patches this issue by adding ``smudging error'' to $c1 \cdot skEnc$:
    instead of sending
    $c1 \cdot [skEnc]$, a committee member sends
    $c1 \cdot [skEnc] + [e_{smudging}]$ to the aggregator.
The addition of smudging error makes the scheme
    provably secure~\cite{asharov2012multiparty,chen2019efficient} (Appx.~\S\ref{sssec:decrypt}) if
the coefficients of the smudging polynomial are 
     from a uniform distribution whose range is much larger
    than the bound of the coefficients of $e_{small}$.
    







    

The addition of $e_{smudging}$, however, raises two questions: 
    how should each committee member obtain 
    its share of $e_{smudging}$, and
    how should \sys obtain
    the bound $B$ of the coefficients of $e_{small}$?
To address the first issue, for each coefficient of $e_{smudging}$, 
    the committee follows
    the standard technique of distributively sampling a random 
    number.

To address the second challenge\label{s:design:derive_B}, we observe that
the error $e_{small}$ grows with ciphertext additions (the error gets added). The bound 
    of 
    a coefficient of $e_{small}$ is therefore a deterministic 
    function of the number of these additions.
If the bound of a coefficient in the 
    $e_{small}$ of a freshly encrypted ciphertext is $B_{fresh}$,
    then after $K$ additions a coefficient is at most
   $B_{fresh}\cdot K$.
Since a committee member knows an upper bound of $K$, which is 
    the maximum number of devices whose data is
    added in the add phase (%
    $M_{max}$ in Figure~\ref{f:addphase}),
it can derive $B$.


%


==> outline.tex <==
\clearpage
\section{Outline}
\subsection{Introdcution}
Cross-device FL is motivated and the models usually have millions of parameters.

To ensure privacy in cross-device FL, we need to have the following two for the system: no trusted core + DP. Reasons are i) inference attacks are possible and DP is a golden privacy guarantee; ii) a malicious server may break user privacy by example attacks.

There are LDP systems, but accuracy is not good. There are systems that assumes trusted cores. The problem is the aggregator can easily break privacy and compromise sensitive information. Even semi-honest is not enough.

Orchard is a general-purpose system that supports full-batch training in the CDP setting (for better accuracy) for small models while meeting the privacy goals: no trusted core + DP. Orchard follows collect-and-test approach: it first collects encrypted data, aggregates the data; devices verify the aggregator work; committee of devices decrypts and adds DP noise inside MPC before releasing the results.

Orchard doesn't scale to models with 1M parameters because of high overhead. give some numbers. the bottlenecks are devices verifying the aggregation needs to download many CTs; releasing the data requires decryption and adding DP noise inside MPC.
The bottlenecks are two types of devices: devices who verify aggregator's work and committee devices who decrypt and add DP noise inside MPC.

\sys starts from Orchard because of its nice threat model. \sys improves Orchard by first picking FedAvg  and then tuning the secure aggreation protocol for it.

\sys uses a new fine-grained verifiable aggregation protocol that i) distribute verification work among more devices; ii) \sys optimizes the cost by PIT fundamentally.

\sys leverages the characteristic of FedAvg to decouple decryption and adding DP noise. \sys have different committees responsible for different committee tasks and use specialized protocol for each task instead of one committee doing all in general-purpose MPC.

How we implements \sys and how we evaluates \sys.
%

\subsection{Background}
\subsection{Problem and threat model, assumption}
introduce FL in general: devices train model; upload updates; aggregator aggregates the updates and update the global model.

introduce possible attacks to FL, for example, a malicious aggregator include one client's data more than once; a malicious client uploading arbitrary gradients, etc.  A malicious client can either deviate from the protocol or go offline.
%

To defend against attacks, the OB+MC threat model is proposed. explain what this threat model. %


\subsection{goals}
1. privacy (introduce DP also)

2. correctness

3. Efficiency and scalability
%

\subsection{existing solutions}
1. straw man solutions: trusted aggregator (secure hardware); it assumes trusted cores, which breaks our privacy goals.

2. straw man solutions: large-scale MPC; it is too expensive and breaks our efficency goals.

3. Orchard

Orchard is internally a secure aggregation protocol, which sums updates from devices.
Present the overview of Orchard's solution. \textbf{maybe use a figure to show it.} % 
\begin{itemize}
    \item setup phase: form the committee; generate keys;
    \item generate phase: generate encrypted uploads and proofs.
    \item add phase: commit; upload; verify
    \item release phase: decrypt, add DP noise.
\end{itemize}

Talk about the bottlenecks under the threat model.
\begin{itemize}
    \item committee devices need to generate fresh keys each round. simply reusing the keys leads to attacks.
    \item verifier devices need to download many ciphertexts to verify the aggregation.
    \item committee devices need to decrypt ciphertexts inside MPC, which involves expensive rounding operations. This is necessary because of their way to add DP noise -- SVT.
\end{itemize}

\subsection{challenges}
scaling Orchard is not easy and the reason is subtle changes might lead to privacy issues. For example, reusing the key looks good in one round of training but lead to attacks in following rounds. Having multiple committees sounds an idea. However, without increasing committee size, this leads to increase of failure probability. Once increasing committee size, the operations will be more expensive. Also decrypting one CT can't be divided for different committees and it's still impractical.

\subsection{overview of \sys}
\subsection{DP-FedAvg}
\sys is designed to support DP-FedAvg. Explain a little bit about why we pick DP-FedAvg. Explain the two characteristics of DP-FedAvg: i) random sampling; ii) independence of gaussian noise (which is different from in Orchard).

DP-FedAvg + Orchard doesn't solve problems.

First, simply applying sampling can lead to less average cost per device. For a single client, with high probability, it does nothing. However, when it is selected to do some work (worst-case cost), the cost will be too expensive. One will need a finer-grained protocol to distribute the verification.

Second, simply replacing SVT with gaussian noise won't solve the problem. Gaussian noise is added inside MPC and the decryption still happens in general MPC. Each rounding operation takes xx MiB and still far too expensive. Also, in each round, a new key pair needs to be generated and this incurs 1 GiB per committee device.
%

\subsection{arch of \sys}
talks about the arch of \sys. \sys has devices, aggregator and three types of committees.

the difference: \sys split the committee work into different tasks and specialized protocol for them.

\subsection{\sys}

\begin{itemize}
    \item setup phase: similar in Orchard, committee needs to generate keys. but \sys i) generate the keys once and ii) reuse/reshare the keys. Simply reusing the key lead to freshness attacks. We fix this issue by making changes in generate phase.
    Reusing the key uses a key resharing protocol instead of generating the key in general MPC and is much more efficient.
    \item generate phase: similar in Orchard, devices locally generate (encrypted) updates and zkproof. Difference: gaussian noise committee + patching the freshness issue (we use a specialized DP noise addition protocol) + sampling. Orchard can't do this since they use SVT to add the DP noise.
    Similarly, generating gaussian noise inside MPC is expensive.
    
    \item add phase: similar in Orchard: aggregator aggregates the updates. Difference: fine-grained trees enables distributing verification work (the failure probability is not impacted); PIT to fundamental improves the cost by 3x. This also reduces the "worst-case" cost, since the clients at least need to verify one tree and that is 18 nodes. (we can't be more fine-grained than one tree containing one CT)
    
    \item release phase: similar in Orchard: committee decrypts and release the results. Difference: DP noise is not added here; we use a specialized decryption protocol instead of expensive general MPC)
\end{itemize}

%
%


\section{Discussion}
talk about generality of the system: internally secure aggregation protocol; Gaussian noise is the constraint
%




TODOs:
create a figure for Orchard;
change the template for osdi

